Towards Standardizing Affine Frequency Division Multiplexing (AFDM) for Future Wireless Networks

Affine frequency division multiplexing~(AFDM) has emerged as a compelling waveform candidate for future wireless networks, owing to its strong resilience to doubly selective channels and its ability to enable the seamless integration of communication and sensing functionalities. Against this context, this article provides a systematic study of AFDM from a standardization perspective. We first introduce the principles of AFDM and discuss the major considerations involved in waveform standardization. We then examine the backwards compatibility of AFDM with 4G/5G multi-numerology frameworks and their anticipated evolution, frequency-modulated continuous-wave (FMCW) radar waveforms, and long-range (LoRa) modulation, demonstrating that AFDM can be incorporated into legacy processing chains with limited modification. Key standardization-critical capabilities are further discussed, including multiple-antenna and multi-user support, and peak-to-average power ratio (PAPR). Finally, we investigate the potential of AFDM in several emerging scenarios, including non-terrestrial networks~(NTN), integrated sensing and communications (ISAC), vehicle-to-everything (V2X), and underwater acoustic (UWA) communications, whereby severe delay-Doppler dispersion places stringent demands on waveform robustness. Through these explorations, it is shown that that AFDM represents a timely and compelling technology for future wireless networks.

==> proposal.tex <==
## 2.2.4 Sensing Approach 4 — AFDM Sensing Using Dedicated Sensing Signal

AFDM is a chirp-based multicarrier waveform in which data symbols are mapped onto orthogonal chirp subcarriers via the Inverse Discrete Affine Fourier Transform (IDAFT). For an AFDM symbol of $N$ subcarriers, the $n$-th discrete-time chirp subcarrier is expressed as:
$$
\psi_n[m] = \frac{1}{\sqrt{N}}\, e^{j2\pi \left(c_1 n^2 + c_2 m^2 + \frac{nm}{N}\right)}, \quad m, n = 0, \ldots, N-1
$$
where $c_1$ imposes a uniform chirp rate across all $N$ subcarriers and $c_2$ introduces subcarrier-dependent initial phases. Each subcarrier $\psi_n[m]$ is obtained by sampling the continuous-time chirp signal $K_n(t) = \frac{1}{\sqrt{N}} e^{j2\pi\!\left(\frac{c_1 N^2}{T^2} t^2 + \frac{n}{T} t + c_2 n^2\right)}$ at the sampling rate $B$, where $T = N/B$ is the symbol duration and $B$ is the system bandwidth. Unlike conventional OFDM subcarriers that occupy a narrow frequency bin, each AFDM chirp subcarrier sweeps linearly across the entire system bandwidth within one symbol duration, providing inherent pulse-compression capability. Notably, OFDM and OCDM are both special cases of AFDM, corresponding to $c_1 = c_2 = 0$ and $c_1 = c_2 = -1/(2N)$, respectively.

When the $N/2$-th subcarrier is activated with $c_1 = 1/(2N)$, the resulting time-domain waveform is equivalent to a digitally-generated FMCW-like chirp, spanning from $-0.5B$ to $0.5B$ with chirp rate $\alpha = B/T$. This section discusses the key properties of AFDM that make it a compelling candidate for dedicated sensing signal design.

---

**Observation 2.2.4-1.** AFDM with a dedicated sensing subcarrier is equivalent to a digitally-generated FMCW waveform, enabling backward compatibility with existing FMCW radar receivers and avoiding strict full-duplex operation.

- AFDM generates chirp waveforms in the digital baseband domain through DAFT-domain modulation, and can be regarded as a Nyquist-sampled discrete-time realization of an FMCW-like chirp. When the $N/2$-th subcarrier is activated with $c_1 = 1/(2N)$, its discrete-time expression reduces to:
$$
\psi_{N/2}[m] = \frac{1}{\sqrt{N}} e^{j2\pi\!\left(\frac{c_1 N^2}{4} + c_2 m^2 + \frac{m}{2}\right)}, \quad m = 0, \ldots, N-1
$$
  where $c_1 = 1/(2N)$. The corresponding continuous-time signal is $K_{N/2}(t) = \frac{1}{\sqrt{N}} e^{j2\pi\!\left(\frac{c_1 N^2}{T^2} t^2 + \frac{N}{2T} t + c_2 \frac{N^2}{4}\right)}$, whose instantaneous frequency $f(t) = \frac{2c_1 N^2}{T^2} t + \frac{N}{2T}$ sweeps linearly from $-B/2$ to $B/2$ over the symbol duration $T$ with chirp rate $\alpha = 2c_1 N^2/T^2 = B/T$. This is precisely the waveform of a conventional FMCW chirp, confirming that the AFDM dedicated sensing subcarrier is digitally equivalent to a full-bandwidth FMCW waveform.

- At the receiver side, the echo signal can be processed using the standard FMCW dechirping architecture: the received echo is mixed with a local reference chirp, producing a beat-frequency (BF) signal whose frequency $f_{\mathrm{BF}} = \alpha\tau$ is proportional to the target range delay $\tau$. Target Doppler can be further estimated from the phase evolution across multiple AFDM symbols, in the same manner as conventional FMCW radar.

- This backward compatibility with FMCW radar signal processing allows the receiver to reuse existing FMCW radar hardware (mixer, LPF, ADC, range FFT), thereby avoiding the stringent self-interference cancellation requirement of full-duplex operation. This is particularly attractive for vehicle, UAV, and IoT platforms where full-duplex capability is difficult to achieve.

- AFDM generates chirps digitally rather than via analog VCO/PLL sweeping, offering finer parametric control, better phase coherence, and seamless integration with the digital communication transceiver chain.

---

**Observation 2.2.4-2.** The chirp-subcarrier structure of AFDM offers a higher degree of freedom for dedicated sensing resource allocation compared to OFDM-based sensing.

- A distinctive property of AFDM is that each chirp subcarrier $\psi_n[m]$ occupies the entire system bandwidth $B$ in the time domain (rather than a narrow sub-band as in OFDM). Consequently, even a single dedicated sensing subcarrier effectively exploits the full bandwidth for range estimation, achieving performance comparable to a full-bandwidth FMCW waveform.

- When deploying a dedicated sensing signal, only one or a small number of AFDM subcarriers need to be assigned as sensing resources, while the remaining subcarriers are freely allocated to communication data and guard intervals. This provides much greater flexibility in communication–sensing resource partitioning compared to OFDM, where a dedicated sensing signal would typically occupy a contiguous sub-band and directly sacrifice spectral efficiency.

- The power allocated to dedicated sensing subcarrier(s) can be independently adjusted according to sensing performance requirements, without affecting the modulation structure of communication subcarriers.

- Deterministic dedicated sensing subcarriers also simplify waveform coordination in bistatic and multistatic deployment scenarios, where the transmitter and receiver are spatially separated or where multiple distributed nodes cooperate for sensing.

---

**Observation 2.2.4-3.** AFDM supports joint time-domain dechirping and DAFT-domain processing, enabling cross-domain signal fusion that can further enhance sensing performance.

- In the time domain, the AFDM dedicated sensing signal is inherently chirp-like, and conventional FMCW dechirping can be directly applied to extract range information via the beat-frequency signal $f_{\mathrm{BF}} = \alpha\tau$. This provides a low-complexity, hardware-efficient sensing path compatible with legacy radar receivers.

- In addition to time-domain dechirping, the DAFT-domain representation of AFDM provides a structured delay–Doppler channel characterization. Target parameters (range, velocity) can alternatively be estimated by time- or DAFT-domain matched filtering after canceling the known sensing waveform. The DAFT-domain processing is particularly amenable to separating multiple targets with distinct delay–Doppler signatures.

- These two processing paths are complementary and can be combined to further improve sensing performance: time-domain dechirping provides coarse range estimation with low complexity and no full-duplex requirement, while DAFT-domain processing enables finer delay–Doppler resolution and multi-target discrimination. Such cross-domain fusion is a unique capability of AFDM that has no direct counterpart in OFDM-based sensing.

- For sensing-centric deployment with larger chirp rates (i.e., $c_1 = Q/(2N)$, $Q > 1$), chirp-fusion schemes (per-symbol segment fusion or cross-symbol BF signal combining) can be applied to preserve FMCW compatibility while accommodating the AFDM CPP structure.

---

**Observation 2.2.4-4.** AFDM exhibits lower range–Doppler sidelobe levels compared to OFDM under high-mobility conditions, making it better suited for sensing in high-speed scenarios.

- In OFDM-based sensing, Doppler shifts caused by high-speed targets destroy subcarrier orthogonality, leading to inter-carrier interference (ICI) that manifests as elevated sidelobes in the delay–Doppler domain and degrades target detection performance.

- AFDM's chirp subcarriers are intrinsically robust against large Doppler spreads. With appropriate chirp parameter selection (i.e., $c_1$ and $c_2$ matched to the expected delay–Doppler spread), AFDM yields a quasi-static and separable effective channel representation in the DAFT domain,
